SKG: A Versatile Information Retrieval and Analysis Framework for Academic Papers with Semantic Knowledge Graphs

The number of published research papers has experienced exponential growth in recent years, which makes it crucial to develop new methods for efficient and versatile information extraction and knowledge discovery. To address this need, we propose a Semantic Knowledge Graph (SKG) that integrates semantic concepts from abstracts and other meta-information to represent the corpus. The SKG can support various semantic queries in academic literature thanks to the high diversity and rich information content stored within. To extract knowledge from unstructured text, we develop a Knowledge Extraction Module that includes a semi-supervised pipeline for entity extraction and entity normalization. We also create an ontology to integrate the concepts with other meta information, enabling us to build the SKG. Furthermore, we design and develop a dataflow system that demonstrates how to conduct various semantic queries flexibly and interactively over the SKG. To demonstrate the effectiveness of our approach, we conduct the research based on the visualization literature and provide real-world use cases to show the usefulness of the SKG. The dataset and codes for this work are available at https://osf.io/aqv8p/?view_only=2c26b36e3e3941ce999df47e4616207f.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January 2022

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> archived_tex/introduction_v1.tex <==
\section{Introduction}

% Prof.Shen: ``One possible motivation for KG is: traditional information retrieval methods are based on the text features, while in real-world applications, users often retrieve information in demand with prior knowledge. This motivates the utilization of knowledge graph in performing information-retrieval tasks from large corpus, which can easily integrate heterogenous information."
% Information retrieval (IR) is the process of representing, storing, and searching through a large collection of text data. 



% This wealth of information presents new opportunities for research studies but also poses new challenges in scientific information retrieval (SIR). 
% First, the relationships between documents can be intricate and diverse, encompassing both structural and semantic relationships, such as citations and semantic similarity. 
% However, extracting, storing, and utilizing these meaningful relationships poses a significant challenge. 
% Additionally, users may struggle to navigate through a large volume of diverse information, making it difficult for them to make informed decisions.  Effectively helping users extract useful information from corpus is a non-trivial task. 

% There have been many efforts across multiple disciplines to address the challenges mentioned above. 
% In the field of text mining, various tasks and technologies have been proposed and developed for text analysis. For example, the methods for solving the classic problem of ranked document retrieval have evolved from using lexical features to neural networks. These methods aim to answer the question of \textbf{``what to read"} by identifying a list of relevant papers from a user's query. 
% More advanced tasks, such as reading path generation, have also been proposed to answer the question of \textbf{``how to read"} by providing a reading order for relevant papers. 
% However, these existing works do not fully utilize all available information. They either only use the structural information, such as citation links, or only consider semantic content as a single source without diving into details. 
% We believe that with the advancements in NLP, the next step is \textbf{``read it for me"} by automatically processing the semantic content and integrating it with other types of information. 

% In the field of visualization, various interactive visual systems have been designed and developed for text analysis. For example, some interactive visual analytics (VA) system incorporates user interactions into algorithms to achieve interactive topic modeling~\cite{kim2020architext, kim2016topiclens}. Other  systems rely on user queries to perform information retrieval from large corpora~\cite{tu2022phrasemap, qiu2022docflow}. However, existing VA systems only address one specific text relationship, neglecting other rich resources and failing to address different kinds of tasks. 


% First, due to the recent development in Natural Language Processing, we believe the information should support more advanced tasks in scientific IR. The tasks have evolved along with the technologies. The most traditional task is document retrieval, to identify a list of relevant papers given users' queries, such as Google Scholar. Later, researchers realized solving ``what to read" is not enough and proposed ``how to read" by recommending a reading path of retrieved documents. 
% The traditional task in scientific IR is to retrieve a list of relevant papers given users' queries, such as Google Scholar. 
% First, the existing tasks in scientific IR are either focused on the structural information of documents, e.g., citation analysis or semantic information, such as document retrieval. However, both resources are useful and informative, which should be integrated and analyzed together to facilitate various tasks and support the data-driven decision-making process. 
% Second, due to the large volume and heterogeneity of the information, how to present the information clearly and interactively is not a trivial problem. 

% brings more challenges in IR.  ``The huge amount of text that is available online is becoming ever increasingly multilingual,
% providing an additional wealth of useful information. "

A knowledge graph (KG) is a graph-based representation of a knowledge base, where entities are represented as nodes and relationships between them are represented as edges. 
Public knowledge graphs, such as DBPedia, Google Knowledge Graph, and YAGO, have shown great performance in various tasks due to their ability to capture diverse information. 
For example, the Google Knowledge graph is used to enhance the search experience by providing users with more relevant and informative search results. 



Incorporating a knowledge graph can bring significant benefits to scientific information retrieval (IR). Traditional IR methods rely on ranking document similarity to user queries based on text features like word frequencies and semantic embeddings. However, these methods may not always fulfill retrieval tasks in real-world scenarios. For instance, a new researcher may need to compare research topics and trends across multiple top conferences to find the most suitable one to submit their work, or an Editor-in-Chief (EIC) may have to compare the research interests of several Associate EIC to assign papers to reviewers.
To overcome these limitations, incorporating knowledge graphs in IR can effectively integrate various types of information from large academic corpora, including citation relationships, semantic relationships, co-authorship, and more. This approach can result in a more efficient and flexible scientific IR.



However, incorporating knowledge graphs into scientific information retrieval presents several challenges. Firstly, it requires a large collection of publications with rich meta-information to ensure the informativeness and usefulness of the knowledge graph. In particular, the knowledge graph must not only contain metadata, such as publication data, conference, year, and authors, but also semantic text data with useful information about the work.
Secondly, extracting and summarizing knowledge from a vast corpus demands significant human effort. Although sub-tasks like entity extraction and relation extraction have been proposed in the field of Natural Language Processing (NLP), these supervised training methods may not be well-suited for scientific publications with out-of-vocabulary issues. A more general solution for all scientific literature is needed to benefit a wider audience.
 % While many existing works have created domain-specific knowledge graphs, such as the ``Internet of Food," ``Food Flow," ``Cultural Historical Community," and ``COVID-19 Knowledge Graph," 
Third, effectively interacting with the academic knowledge graph to generate insights efficiently poses significant challenges. Efforts from multidisciplinary domains are being made to address this issue. 
In Natural Language Processing (NLP), many sequence-to-sequence models have been proposed to translate natural languages into structured queries to query the knowledge graph, such as Cypher and SPARQL. However, there is a high learning curve to learn the semantics and schema of these languages. Testing and debugging generated queries may also interrupt the continuity of data analysis and information retrieval. 
In visualization, there are some interactive systems developed to facilitate the interaction with knowledge graphs~\cite{xiao2019virtual}, including entity summarization~\cite{wei2020vision,qiu2020tax}, recommendation~\cite{shao2021survey}, question answering~\cite{calvanese2011mastro,priyatna2014formalisation}, query formulation~\cite{soylu2018optiquevqs,ferre2017sparklis}, and ontology curation, Protégé~\footnote{\url{https://protege.stanford.edu}}, IDE Stardog Studio~\footnote{\url{https://www.stardog.com/studio}}. However, they do not directly target scientific information retrieval tasks, which are in great need of such systems. 


% In this work, to enable knowledge-driven Scientific IR, we propose an approach that combines natural language processing technologies and visual analytics.
% Our approach involves two key steps, corresponding to addressing two aforementioned challenges. 
% First, to 
In this work, we propose an approach to achieve interactive knowledge-driven information retrieval in academics and demonstrate the approach in \emph{visualization} literature. Our approach involves several key steps, aiming to address the  aforementioned challenges accordingly. 
First, to ensure a large volume and high diversity of information for knowledge graph construction, we create a new dataset called \emph{$\DATABASE$}, which consists of $125,745$ papers from the visualization literature. The $\DATABASE$ dataset contains paper information, such as the title, authors, and publication details, as well as structural information, such as citations and co-author relationships. 
However, translating such a dataset into a heterogeneous knowledge graph is challenging when extracting semantic entities from raw paper text. To overcome this, we propose a pipeline that performs named entity recognition (NER) and entity normalization from paper abstracts. 
To address the challenge of preparing a training dataset for the NER task, which involves a large labeling workload, our pipeline employs a semi-supervised approach.
We use a pre-trained language model to generate weak training samples, which are then filtered and annotated by human annotators as a high-quality training dataset. 
The structured semantic entities, along with other meta-information, are integrated into an academic knowledge graph in the visualization literature. 
Furthermore, to achieve knowledge-driven information retrieval, we build a dataflow system that allows users to interact with the constructed knowledge graph. We identify several basic tasks users may want to perform and abstract them into visual operations. We then design several components with specified inputs/outputs, which users can drag and drop to build different analysis pipelines to fulfill various tasks.
This allows users to explore the dataset quickly and gain insights from it.
In short, our contributions can be summarized as follows:
\begin{itemize}
    \item We prepare a dataset, $\DATABASE$, which includes $125,745$ papers from various sub-areas of the visualization literature. The dataset is publicly available on: \red{TBA}, and has the potential to benefit the literature in numerous ways. 
    \item We propose a general semi-supervised pipeline for constructing academic knowledge graphs that can be easily transferred to other scientific domains. The constructed knowledge graph in the visualization literature can also benefit many downstream tasks, such as question answering and neural embedding generation.
    \item We have also designed and developed a dataflow system for scientific information retrieval. We demonstrate the system's usefulness and effectiveness through several real-world usage scenarios.
\end{itemize}
% Some visual graph query methods are proposed to allow users to construct the query by adding node or link. 
% it is required to learn the visual programming langauge 
% it is tedious to construct the query 

% the massiveness, heterogeneity, dynamics, and diversity of Web data have
% become the major challenges facing information retrieval.

% Autocompletion 




==> archived_tex/method_v1.tex <==
% \section{Requirement Analysis}
% We aim to construct a domain-specific knowledge graph in the visualization literature to help downstream tasks. To accomplish this, we have been holding weekly meetings with domain experts to discuss the requirements of the knowledge graph. 
% After conducting a literature review and consulting with the expert, we have summarized the requirements as follows:


% \begin{itemize}
%     \item \textbf{R1.Multi-faceted Information}. While some academic knowledge graphs include structural information, such as citations, integrating semantic information can facilitate more advanced text analysis tasks that require reading comprehensions, like summarization and recommendation. 
%     \item \textbf{R2.Minimal Human Labeling Effort}. Building a knowledge graph from scratch requires extensive data cleaning, and human labeling. To cope with the growing number of publications, the method should leverage machine readability and minimize human labor. Additionally, it should ensure the approach can be easily transferred to other domains and scalable to new corpora.
%     \item \textbf{R3.Adherence to FAIR principles.}
%     The knowledge graph should be designed following the FAIR guiding principles for scientific data management, ensuring that digital assets are \textbf{F}indability, \textbf{A}ccessibility, \textbf{I}nteroperability, and \textbf{R}euse of digital assets. 
%     % \red{Dataset}
%     \item \textbf{R4.Intuitive Support for Downstream Tasks}. The constructed KG should support various tasks in scientific information retrieval, such as document retrieval, literature review, topic modeling, and reviewer finding, in an intuitive and flexible manner. 
%     % \red{System}
% \end{itemize}

\section{Method}
 We have developed a method that combines natural language processing (NLP) techniques with visual analytics to facilitate semantic queries in the academic literature. Our approach consists of four components, as depicted in \autoref{fig:overview}. We first present an overview of our approach and then introduce each component in detail. 


\subsection{Approach Overview}

To expand the scope of knowledge in the VIS literature, a wealth of scientific publications with rich information in this field is necessary (\textbf{R1}). 
While there exist some databases in the VIS literature, they can not be directly utilized to build our knowledge graph for two reasons: (1) they mainly focus on specific conferences or journals, omitting other critical sub-areas, such as VisPub ~\cite{isenberg2016visualization}. 
(2) they fail to capture the structural relationship among documents. For instance, VitaLITy~\cite{narechania2021vitality} does not contain the citation relationship among documents, which can decrease the informativeness of the constructed knowledge graph and fail to perform relevant tasks. To overcome these limitations, we construct a new dataset called $\DATABASE$, which contains $14,6130$ papers in the VIS literature with both semantic and structural information.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/overview.pdf}
    \caption{An overview of our approach involves four main steps: (1) constructing a new dataset called $\DATABASE$ by collecting data from various sources, (2) performing knowledge reasoning from unstructured textual data, (3) building the knowledge graph, and (4) constructing a dataflow system to interactively query the knowledge graph.}
    \label{fig:overview}
\end{figure}


Building the knowledge graph from unstructured textual data automatically is not a trivial task. To extract useful knowledge from the textual content of papers with minimal human labeling (\textbf{R2}), we build a \emph{knowledge extraction pipeline} in a semi-supervised manner to perform entity definition, recognition, and alignments from $\DATABASE$. 

One big effort in promoting the FAIR principle is Linked Open Data, which aims to link the data on the Internet from various sources (\textbf{R3}). 
Resource Description Framework (RDF) is a commonly used data structure to achieve the Linked Open Data, representing knowledge as \textit{triplets}. Based on well-known academic knowledge graphs, such as Microsoft Academic Knowledge Graph (MAKG),  we carefully design an ontology and construct an RDF knowledge graph using it. 


Driven by \textbf{R4}, we design and develop a data flow system to demonstrate how the knowledge graph can enhance various information retrieval tasks. 
We offer several standard components with pre-defined input/output and functionality that enable users flexibly construct their query and analysis pipeline flexibly to interact with the knowledge graph. 
% \begin{itemize}
%     \item \textbf{Data Preparation:} We outline our process of gathering papers in the VIS literature by leveraging various online sources. 
%     \item \textbf{Knowledge Graph Construction:} We constructed a knowledge graph based on a domain-specific ontology to model multi-faceted information. This involved integrating concepts from different perspectives along with additional meta-information. 
%     \item \textbf{Interactive KG Querying:} We designed and developed a data flow system that enables interactive querying and analysis of data from the knowledge graph, demonstrating its usefulness for information retrieval and gaining insights.
% \end{itemize}
 

% Knowledge graphs (KG) provide rich abstractions for addressing data heterogeneity. 
% In this work, the aim of breaking the boundaries of knowledge, we construct an 
% an academic KG in the VIS literature. 
\subsection{The $\DATABASE$ Dataset }
We introduce the $\DATABASE$ dataset, utilized for us to construct a knowledge graph in VIS literature. We first provide an overview of the dataset and then introduce the construction process.

\subsubsection{Overview of $\DATABASE$}
The goal of the $\DATABASE$ is to offer comprehensive information on publications in the VIS literature that satisfies two key criteria: (1) it should include a diverse range of sub-areas of the VIS literature, and (2) it should  capture both meta-information such as \emph{title}, \emph{venue}, \emph{year}, and structural relationships among publications, such \emph{co-author}, \emph{citation}, as well as the semantic information, i.e., \emph{abstract}.

The $\DATABASE$ comprises $125,745$ papers from the VIS literature. 
We use the same format as the Semantic Scholar Open Research Corpus (S2ORC)~\cite{lo-wang-2020-s2orc} dataset, which includes 25 attributes. 
\autoref{tab:visbank}A provides the number of papers missing specific attributes.
Specifically, all papers in the $\DATABASE$ have a \emph{title}, but $18,591$ papers are missing an \emph{abstract}, $430$ papers do not include \emph{author} information, and $902$ papers do not include \emph{venue} or \emph{journal} information. 

We compare the $\DATABASE$ to two well-known academic datasets in the VIS literature, i.e., \emph{VisPub} and \emph{VitaLITy}, and the results are shown in   \autoref{tab:visbank}B. 
The coverage of both datasets by our $\DATABASE$ reaches $89\%$, which suggests that our dataset not only covers and merges existing resources but also includes additional rich information. 
Also, the paper distribution across sub-areas in the VIS literature is shown in \autoref{tab:visbank}C, highlighting the multidisciplinary nature of the VIS field that encompasses various research topics beyond visualization, including human-computer interaction, knowledge and data extraction, virtual reality, and more.
Additional details regarding related journals and venues can be found in the supplemental material. 


% Comparing the $\DATABASE$ with the 
\subsubsection{Dataset Construction}
We construct the $\DATABASE$ based on the S2ORC dataset since (1) captures metadata and paper text information; (2) contains 136 million papers from various fields of study.  The construction pipeline has several steps:

\textbf{Filter Field of Study}. 
The original S2ORC corpus contains over 136 million scientific papers across a variety of fields, including medicine, biology, physics, and others. 
In order to identify papers within the field of visualization, we first restrict the field of study to 
 \texttt{computer science} only, which results in a total of 12 million papers. 

\textbf{Identify Sub-Fields in VIS}
To identify the relevant papers of sub-fields as shown in \autoref{tab:visbank}C, we perform a keyword-based search. For example, we use the keyword ``visualization" to identify related journal and venue names such as \emph{TVCG}, \emph{Journal of Visualization}, \emph{Volume Visualization} and etc.
By using this approach, we have compiled a full list of $3520$ relevant venues and $88$ journals, which can be found in the supplemental material. 

\textbf{Filtering and Merging}
By filtering on the venue and journal, we get $87,246$ papers from the S2ORC. 
Given the high quality of the S2ORC dataset, we also map papers from \emph{VisPub} and \emph{VitaLITy} to the S2ORC by matching titles, merging the three sources, and removing all the duplicate items to form the $\DATABASE$. 
The final dataset contains $125,745$ papers. 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\small
\setlength{\tabcolsep}{1pt}
\begin{tabular}{l|lr|l|lr}
\hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}(A)\\ Statistics \\ of missing\\ attr.\end{tabular}}} & No Title & 0 & \multirow{8}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}(C)\\ Sub\\ Area\end{tabular}}} & Graphics \&Visualization & 55,759 \\
 & No Abstract & 18,591 &  & Human-Computer Interaction & 36,719 \\
 & No Author & 430 &  & Knowledge \& Data mining & 9,490 \\
 & No Venue/Journal & 902 &  & Virtual/Augmented Reality & 7,648 \\
 & Total & 125,745 &  & Cognitive Science & 6,514 \\ \cline{1-3}
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}(B)\\ Compare\end{tabular}}} & VisPub & 3,120/3,503 &  & Ubiquitous Computing & 4,524 \\
 & VitaLITy & 52,784/59,232 &  & User Interaface, System & 2,279 \\
 & S2ORC & 125,745/135M &  & Others & 2,812 \\ \hline
\end{tabular}
\caption{Statistical information regarding the $\DATABASE$ dataset includes (A) the number of publications that are  missing specific attributes; (B) a comparison of the $\DATABASE$ with other datasets in the VIS literature; (C) The paper distributions across sub-areas in the VIS literature. }
\label{tab:visbank}
\end{table}
% https://arxiv.org/pdf/2108.03366.pdf
% \subsection{The VisSurvey Dataset}
% In this section, we introduce the VisSurvey Dataset to evaluate our RMG task. We provide an overview of the dataset, describe the construction pipeline, and present some statistical analysis to demonstrate its quality.
% % \subsection{Overview}
% why do we need this dataset?
% 1. vispub only contains inner citations with limited access 
% 2. other do not focus on the Vis literature. 
% % \subsection{Dataset Construction}
% We used the Semantic Scholar Open Research Corpus (S2ORC) to create the VisSurvey dataset. The process of creating the VisSurvey dataset is shown in Figure 1 and consists of three steps. First, we filtered the 12 million papers in the field of computer science out of the 136 million papers and obtained all unique venues and journals. 
% Next, we summarized a set of keywords based on the conference partners of TVCG. Based on keyword matching, we identified relevant venues/journals in the visualization literature and detailed them in \autoref{tab:journal}. 
% Finally, we further filtered the papers and ended up with $107,831$ papers published in vis venues/journals as corpus $\mathcal{D}$. 
% From the corpus $\mathcal{D}$, we locate 86 survey papers by filtering for the word ``survey" in the title, which is used to create the final set $\mathcal{S}$. 

% \subsection{}

% \begin{algorithm}[h]
% \SetAlgoLined
% \KwIn{Knowledge Graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, User-defined Query $q$, step $k$.}

% \KwOut{Subset of paper nodes $\{v | v.type=``makg.paper", v\in \mathcal{V}\}$.}%, with the set of edge attributes Attr(E) = attn\_avg}

% \nl Find a list of nodes $v$ related to $q$ as seeds $\mathcal{S}\in \mathcal{V}$.

% \nl \For{$s \in \mathcal{S}$}{
% \nl Find neighboring paper nodes of $s$ within $k$ hops, denoted as $\mathcal{N}_s$.\\
% \nl \For{$n \in \mathcal{N}_v$}{
%     \nl Find all simple paths $P$ between $v$ and $n$ within $k$ hops. \\
%      \nl   \For{$p \in P $}{
%       \nl      \eIf{$p.type=``makg.paper"$}{
%       \nl          $p.count +=1$
%             }
%         }
%     }
% }
% \nl Sort all nodes $v$ by $count$ and find top rated nodes as recommendations.

% \caption{\bf Constructing PhraseMap for corpus} 
% \label{alg:PhraseMap}
% %   \vspace{-1.5em}
% \end{algorithm}


\subsection{Knowledge Extraction Pipeline}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/semi-supervised.pdf}
    \caption{Knowledge Extraction Module consists of three steps.}
    \label{fig:ner}
\end{figure*}

Converting unstructured text into a structured knowledge graph is a challenging task due to the inherent complexity of natural language.
To extract entities and their semantic relationship from scientific paper abstracts, we propose an ontology-based semi-supervised pipeline for entity extraction, classification, and alignment.

% \subsubsection{Entity Class Definition}
Before introducing our pipeline, we rigorously define the semantic entities extracted from the paper abstracts. 
Prior academic literature defines four sub-domains of knowledge in abstracts as  
$<\textit{background}, \textit{objective}, \textit{method}, \textit{result}>$~\cite{chen2019automatic, cohan2019pretrained}.
Since our focus is on the visualization domain, we modify the definition by adopting the sub-category of keywords used in IEEE VIS, one of the top conferences in the field. 
We define extracted entity $e$ as belonging to one of five sub-domains: $<$\textit{data, application, method, visualization, evaluation}$>$. In other words, the label of an entity, denoted $\mathcal{L}(e)$, can be one of $\{l_{d}, l_{a}, l_{m}, l_{v}, l_{e}\}$.

There are several advantages to using our defined sub-domains for organizing semantic knowledge. First, it contributes to the clarity and diversity of the academic knowledge graph we aim to build by organizing knowledge from different perspectives. 
Second, pre-processing knowledge into different perspectives can benefit advanced tasks. For example, in a literature review of text visualization~\cite{liu2018bridging},  summarizing and aggregating papers based on text mining methods and visualization charts can be facilitated by our defined sub-domains. 


To extract entities automatically with our defined labels, we propose a semi-supervised learning framework. 
As shown in \autoref{fig:overview}, the framework comprises three steps: (1) unsupervised learning to generate weak training samples; (2) filtering high-confidence samples and soliciting human annotators to create high-quality training samples; (3) supervised training of a Named Entity Recognition (NER) model. We will explain each step in detail.

\subsubsection{Unsupervised Learning for Weak Samples}
We construct an unsupervised pipeline to generate weak training samples to assist further human labeling: including entity extraction and entity classification. 


Entity extraction from scientific publications typically involves identifying noun n-grams~\cite{zhang2021conceptscope}, such as ``volume rendering". To extract these n-grams, we first generate the Part-of-Speech (POS) tag for each word in the publication, which indicates the grammatical function of the word in the sentence. We then use a rule-based approach to extract the noun n-grams based on the POS tags. This approach has high readability and is easy to tune to achieve high coverage of all entities~\cite{tu2022phrasemap,waltl2018rule}. The set of rules and example entities can be found in the \red{TBA}.


Performing entity classification in an unsupervised manner can be challenging since it is typically a supervised task. However, recent findings in the NLP literature suggest that a single frozen pre-trained language model can be fine-tuned for various downstream tasks. Inspired by this, we propose a novel approach to modify the Question Answering (QA) model pipeline to perform entity classification with fixed pre-trained parameters. 
The high-level idea of our approach is that ask a set of questions related to entity labels for each entity and assign the entity to the label for which it is most likely to answer the corresponding question. 
For example, the \emph{data} label $l_d$ is translated into \textit{what is the data?} or \textit{what is the dataset?}. The full list of labels with translated questions is provided in \autoref{tab:qa_question}. 


In this work, we utilize the fine-tuned QA model, Roberta\footnote{https://huggingface.co/deepset/roberta-base-squad2}, to perform entity extraction. Typically, the input to a QA model is a question with a contextual document $(q, d)$. The model is trained to find the start token $t_s$ and end token $t_e$ of an answer from the document.
The QA model has two sets of trainable weights, $\textbf{W}_S, \textbf{W}_E$, which are used to compute the score of each token $t_i$ being the start token and end token using:
\begin{equation}
      score_S(q, d, t_i) = \frac{e^{{\textbf{W}_S} \cdot \bf{v}_i}}{\sum_{j}e^{{\textbf{W}_S} \cdot  \bf{v}_j}}, \quad score_E(q, d, t_i) = \frac{e^{{\textbf{W}_E} \cdot \bf{v}_i}}{\sum_{j}e^{{\textbf{W}_E} \cdot \bf{w}_j}}.
\end{equation} where $\textbf{v}_{i}$ is the embedding of a token $t_i$, which is an intermediate output in the Roberta sharing the same dimensions with the weights ($768d$). After taking the dot product between token embeddings and the start/end weight matrix, we apply the softmax activation to compute a probability distribution over all tokens. 
To perform entity classification, for each entity $e$, we compute the $score_S$ for its starting token $t_i$ and $socre_E$ for its ending token $t_j$ and assign it to the question $q_m$ with the highest score $S$ as follows:
\begin{equation}
   \argmax_m S= score_S(q_m, d, t_i)\cdot score_E(q_m, d, t_j) 
\end{equation} The score $S$ indicates how likely the entity $e$ can answer the question $q_m$. 
Based on the mapping in \autoref{tab:qa_question}, we assign the corresponding label of the question with the highest score to the entity.  
After this process, we obtain a set of outputs, denoted as (entity $e$, label $l$, score $S$), where each pair indicates one semantic entity $e$ being assigned to label $l$ with the confidence score $S$. For each label $l$, we sort the corresponding samples based on the score $S$ and select top-K as high-confident \emph{weak training samples}. 
 % \frac{e^{(e_i)\cdot $\textbf{W}_s$}}{\sum_{i}e^{(e_i)\cdot $\textbf{W}_s$}
% This approach leverages the ability of pre-trained language models to encode contextual information and make predictions based on it. 
% Then we attach the questions with 
 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\small
\centering
\begin{tabular}{lll}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Label} & \textbf{Notation} & \textbf{Question} \\ \hline
 &  & What is the data? \\
\multirow{-2}{*}{\textbf{Data}} & \multirow{-2}{*}{$l_{data}$} & What is the dataset? \\ \hline
 &  & What is the application? \\
\multirow{-2}{*}{\textbf{Application}} & \multirow{-2}{*}{$l_{app}$} & What is the task? \\ \hline
 &  & What is the method? \\
 &  & What is the algorithm? \\
\multirow{-3}{*}{\textbf{Method}} & \multirow{-3}{*}{$l_{method}$} & What is the technique? \\ \hline
 &  & What is the visualization? \\
\multirow{-2}{*}{\textbf{Visualization}} & \multirow{-2}{*}{$l_{vis}$} & What is the chart? \\ \hline
\textbf{Evaluation} & $l_{eval} $ & What is the evaluation? \\ \hline
\end{tabular}
\caption{TBA}
\label{tab:qa_question}
\end{table}
 
 
 
 % we translate each label into a question and attach it with the 

\subsubsection{Human Annotator Fine-tuning}
We invited human annotators to refine \emph{weak training samples}, which may have arisen from either extraction or classification. We aimed to leverage the strengths of both machines and humans in the annotation process. Machines were utilized to assist in labeling tasks that were easily understood by them, while human annotators were utilized to address the limitations of machine understanding.


We conducted the annotation process iteratively. Initially, we labeled entities following the same principle as in \autoref{tab:qa_question} for question answering. For instance, we labeled entities related to tasks and applications as $l_{app}$. However, during the human annotation phase, disagreements arose between the machine and the human annotators. To resolve these discrepancies, we held discussions with five PhD students who have expertise in visualization. We discussed and agreed upon a proper solution and applied it consistently throughout the annotation pipelines. For instance, we noticed that several entities labeled as $l_{app}$ were incorrectly labeled as $l_{vis}$ by the machines. We analyzed the cause and found that it stemmed from the context, as they typically had the format of ``visualization of data."


We labeled a total of $5076$ samples and converted them into token classification format \footnote{\url{https://huggingface.co/datasets/Yamei/NER_VISBank}} to train our NER model. In this format, each token in a sequence $[t_1, t_2,.., t_i]$ is assigned a label $[l_1, l_2,.., l_i]$. 
In addition, the label $l_i$ for each token is prefixed with $B$ or $I$ to indicate whether the token is the beginning or continuation of an entity respectively. An example is illustrated in \autoref{fig:ner}.
% First, 
% pre-defined rules may fail to extract some rare entities. For example, ``in situ visualization" (FW-FW-NN) fails to be captured, but it is an important concept in visualization. 
% Secondly, the QA model assigns a higher score to a wrong label during to the entity overlapping. For instance, phrases like ``visualization of textual data", the QA model assigns \emph{textual data} to $l_{vis}$ instead of $l_{data}$ 

\subsubsection{NER Training}


% There are some existing machine learning techniques trained to extract the $<\textbf{s}ubject, \textbf{p}redicate, \textbf{o}bject>$
% from English sentences. But they require a set of human-annotated triplets, which is time-consuming and energy-demanding. 
% While other unsupervised methods, such as Standford Parser, can generate triplets based on syntactic information. They can not guarantee a high-quality result and increase the complexity of entity/link alignments. 


\subsection{Graph Construction}


\subsection{Interactive Querying: Data Flow System}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/system.pdf}
%     \caption{Caption}
%     \label{fig:system}
% \end{figure}

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

